Comparing Fixed and Adaptive Computation Time for Recurrent Neural Networks

Adaptive Computation Time for Recurrent Neural Networks (ACT) is one of the most promising architectures for variable computation. ACT adapts to the input sequence by being able to look at each sample more than once, and learn how many times it should do it. In this paper, we compare ACT to Repeat-RNN, a novel architecture based on repeating each sample a fixed number of times. We found surprising results, where Repeat-RNN performs as good as ACT in the selected tasks. Source code in TensorFlow and PyTorch is publicly available at https://imatge-upc.github.io/danifojo-2018-repeatrnn/

==> preamble.tex <==
% Idioma (és important a l'hora de separar una paraula a final de línia)
 %\usepackage[catalan] {babel}
 %\usepackage[spanish] {babel}
 %\usepackage[english] {babel}    
                        
 \usepackage{bbm}                                       % Permet fer \1
            %%% Nota: Si la plantilla no compila, comenta els dos packages anteriors.
 \usepackage{cancel}
 %\usepackage[utf8]{inputenc}                            % Accents i símbols extranys
 \usepackage{amsfonts,amssymb}                          % Símbols matemàtics
 \usepackage[version=4]{mhchem}
 \usepackage{mathrsfs}                                  % Lletra cal·ligràfica (millor que \mathcal)
 \usepackage{amsmath}                                   % Mode matemàtic
 \usepackage{amsthm}                                    % Teoremes
%\usepackage{bookman}                                   % BarreroTimes
 \usepackage{verbatim}                                  % Verbatim + comentaris multilínia
 \usepackage{graphicx,subcaption}                       % Fotos i subfotos
 % \usepackage[free-standing-units]{siunitx}              % Sistema internacional
 \usepackage{float}                                     % Posa les figures on toca
 \usepackage{bm}
 \usepackage{scrextend}
 \usepackage{anysize}                                   % Posa els marges
 \marginsize{2cm}{2cm}{1cm}{4cm}     % {L}{R}{U}{D}
 \usepackage{tikz-cd}                                   % Diagrames commutatius
 \usepackage{float}
 \usetikzlibrary{babel}                                 % Evita interferència entre tikz-cd i babel

%Conjunts importants
\def\NN{\mathbb N}   % Naturals
\def\ZZ{\mathbb Z}   % Enters
\def\QQ{\mathbb Q}   % Racionals
\def\RR{\mathbb R}   % Reals
\def\CC{\mathbb C}   % Complexos
\def\HH{\mathbb H}   % Quaternions, semiplà superior complex
\def\AA{\mathbb A}   % Espai afí en general
\def\EE{\mathbb E}   % Extensió d'un cos, esperança
\def\FF{\mathbb F}   % Cos primer, cos finit
\def\KK{\mathbb K}   % Cos en general
\def\PP{\mathbb P}   % Espai projectiu, nombres primers
\def\DD{\mathbb D}   % Disc unitat complex
\def\SS{\mathbb S}   % Esfera
\def\TT{\mathbb T}   % Tor (n-dimensional)

% Per escriure menys
\def\oo{\infty}                                         % Infinit
\def\P{\mathscr P}                                      % Conjunt potència
\def\A{\mathscr A}                                      % Àlgebra, sigma-àlgebra
\def\B{\mathscr B}                                      % Base
\def\T{\mathscr T}                                      % Topologia
\def\L{\mathscr L}                                      % Espai d'homomorfismes, derivada de Lie
\def\C{\mathscr C}                                      % Funcions contínues, derivables amb continuïtat
\def\D{\mathscr D}                                      % Funcions derivables
\def\mm{\mathfrak M}                                    % Matrius
\def\ss{\mathfrak S}                                    % Grup simètric
\def\aa{\mathfrak A}                                    % Grup alternat
\def\Re#1{\mathfrak {Re}\left\{#1\right\}}              % Part real
\def\Im#1{\mathfrak {Im}\left\{#1\right\}}              % Part imaginària
\def\1{\mathbbm{1}}                                     % Funció indicadora
\def\<{\langle}                                         % subespai/ideal/subgrup -
\def\>{\rangle}                                         % generat per, producte escalar

\def\vphi{\varphi}       %\phi       = SIDA              
\def\vepsilon{\varepsilon}   %\epsilon   = SIDA

\DeclareMathOperator*{\argmin}{arg\,min}                                 % Punt on s'assoleix el mínim
\DeclareMathOperator*{\argmax}{arg\,max}                                 % Punt on s'assoleix el màxim
\DeclareMathOperator*{\mex}{mex}                                         % Mínim ordinal exclòs
\DeclareMathOperator*{\sgn}{sgn}                                         % Signe
\DeclareMathOperator*{\im}{Im}                                           % Imatge
\DeclareMathOperator*{\Tr}{Tr}                                           % Traça
\DeclareMathOperator*{\Id}{Id}                                           % Identitat
\DeclareMathOperator*{\supp}{supp}                                       % Suport
\DeclareMathOperator*{\prolim}{\underleftarrow{\rm{proj\,lim}}}          % Límit projectiu
\DeclareMathOperator*{\indlim}{\underrightarrow{\rm{ind\,lim}}}          % Límit inductiu

%Trigonometria bàsica
\DeclareMathOperator*{\tg}{tg}                          % tg(·)          = sin(·)/cos(·)
\DeclareMathOperator*{\cosec}{cosec}                    % cosec(·)       = 1/sin(·)
\DeclareMathOperator*{\cotg}{cotg}                      % cotg(·)        = cos(·)/sin(·)
\DeclareMathOperator*{\cotan}{cotan}                      % cotg(·)        = cos(·)/sin(·)


\DeclareMathOperator*{\arctg}{arctg}
\DeclareMathOperator*{\arcsec}{arcsec}
\DeclareMathOperator*{\arccosec}{arccosec}
\DeclareMathOperator*{\arccotg}{arccotg}
\DeclareMathOperator*{\arccotan}{arccotan}

\DeclareMathOperator*{\tgh}{tgh}                        % tgh(·)         = sinh(·)/cosh(·)
\DeclareMathOperator*{\sech}{sech}                      % sech(·)        = 1/cosh(·)
\DeclareMathOperator*{\cosech}{cosech}                  % cosech(·)      = 1/sinh(·)
\DeclareMathOperator*{\cotgh}{cotgh}                    % cotgh(·)       = cosh(·)/sinh(·)
\DeclareMathOperator*{\cotanh}{cotanh}                    % cotgh(·)       = cosh(·)/sinh(·)


\DeclareMathOperator*{\arcsinh}{arcsinh}
\DeclareMathOperator*{\arccosh}{arccosh}
\DeclareMathOperator*{\arctgh}{arctgh}
\DeclareMathOperator*{\arctanh}{arctanh}
\DeclareMathOperator*{\arcsech}{arcsech}
\DeclareMathOperator*{\arccosech}{arccosech}
\DeclareMathOperator*{\arccotgh}{arccotgh}
\DeclareMathOperator*{\arccotanh}{arccotanh}

\DeclareMathOperator*{\versin}{versin}                  % versin(·)      = 1-cos(·)
\DeclareMathOperator*{\vercos}{vercos}                  % vercos(·)      = 1+cos(·)
\DeclareMathOperator*{\coversin}{coversin}              % coversin(·)    = 1-sin(·)
\DeclareMathOperator*{\covercos}{covercos}              % covercos(·)    = 1+sin(·)
\DeclareMathOperator*{\haversin}{haversin}              % haversin(·)    = (1-cos(·))/2    = sin^2 (·/2)
\DeclareMathOperator*{\havercos}{havercos}              % havercos(·)    = (1+cos(·))/2    = cos^2 (·/2)
\DeclareMathOperator*{\hacoversin}{hacoversin}          % hacoversin(·)  = (1-sin(·))/2
\DeclareMathOperator*{\hacovercos}{hacovercos}          % hacovercos(·)  = (1+sin(·))/2

\DeclareMathOperator*{\arcversin}{arcversin}
\DeclareMathOperator*{\arcvercos}{arcvercos}
\DeclareMathOperator*{\arccoversin}{arccoversin}
\DeclareMathOperator*{\arccovercos}{arccovercos}
\DeclareMathOperator*{\archaversin}{archaversin}
\DeclareMathOperator*{\archavercos}{archavercos}
\DeclareMathOperator*{\archacoversin}{archacoversin}
\DeclareMathOperator*{\archacovercos}{archacovercos}

\DeclareMathOperator*{\versinh}{versinh}                % versinh(·)     = 1-cosh(·)
\DeclareMathOperator*{\vercosh}{vercosh}                % vercosh(·)     = 1+cosh(·)
\DeclareMathOperator*{\coversinh}{coversinh}            % coversinh(·)   = 1-sinh(·)
\DeclareMathOperator*{\covercosh}{covercosh}            % covercosh(·)   = 1+sinh(·)
\DeclareMathOperator*{\haversinh}{haversinh}            % haversinh(·)   = (1-cosh(·))/2   = -sinh^2 (·/2)
\DeclareMathOperator*{\havercosh}{havercosh}            % havercosh(·)   = (1+cosh(·))/2   = cosh^2 (·/2)
\DeclareMathOperator*{\hacoversinh}{hacoversinh}        % hacoversinh(·) = (1-sinh(·))/2
\DeclareMathOperator*{\hacovercosh}{hacovercosh}        % hacovercosh(·) = (1+sinh(·))/2

\DeclareMathOperator*{\arcversinh}{arcversinh}
\DeclareMathOperator*{\arcvercosh}{arcvercosh}
\DeclareMathOperator*{\arccoversinh}{arccoversinh}
\DeclareMathOperator*{\arccovercosh}{arccovercosh}
\DeclareMathOperator*{\archaversinh}{archaversinh}
\DeclareMathOperator*{\archavercosh}{archavercosh}
\DeclareMathOperator*{\archacoversinh}{archacoversinh}
\DeclareMathOperator*{\archacovercosh}{archacovercosh}

\DeclareMathOperator*{\exsec}{exsec}                    % exsec(·)       = sec(·)-1        = versin(·)sec(·)
\DeclareMathOperator*{\excosec}{excosec}                % excosec(·)     = cosec(·)-1      = coversin(·)cosec(·)
\DeclareMathOperator*{\crd}{crd}                        % crd(·)         = 2sin(·/2)
\DeclareMathOperator*{\arcexsec}{arcexsec}
\DeclareMathOperator*{\arcexcosec}{arcexcosec}
\DeclareMathOperator*{\arccrd}{arccrd}

% Permet fer peus de pàgina amb altres símbols
\makeatletter
\def\@xfootnote[#1]{\protected@xdef\@thefnmark{#1}\@footnotemark\@footnotetext}
\makeatother


% Objectes no textuals
\begin{comment}
--------------------Taula--------------------

    http://www.tablesgenerator.com

-------------Diagrama Commutatiu-------------

    http://osl.ugr.es/CTAN/graphics/pgf/contrib/tikz-cd/tikz-cd-doc.pdf

-------------------Circuit-------------------

    http://texdoc.net/texmf-dist/doc/latex/circuitikz/circuitikzmanual.pdf

--------------------Foto---------------------

    \begin{figure}[H]
        \centering
        \includegraphics[width=\linewidth]{Imatges/Loremipsum.png}
    \end{figure}

-------------------Subfoto-------------------

    \begin{figure}[H]
        \begin{subfigure}[b]{.5\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Imatges/Lorem.png}
        \end{subfigure}
        \begin{subfigure}[b]{.5\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Imatges/Ipsum.png}
        \end{subfigure}
    \end{figure}

\end{comment}

% Per veure si falta res en un treball (el típic "ho deixo per després")
\DeclareMathOperator*{\completar}{\_\_\_\_\_\_\_\_\_\_}
